Visualizing Environmental Justice Issues in Urban Areas with a Community-based Approach

According to environmental justice, environmental degradation and benefits should not be disproportionately shared between communities. Identifying disparities in the spatial distribution of environmental degradation is therefore a prerequisite for validating the state of environmental justice in a geographic region. Under ideal circumstances, environmental risk assessment is a preferred metric, but only when exposure levels have been quantified reliably after estimating the risk. In this study, we adopt a proximity burden metric caused by adjacent hazardous sources, allowing us to evaluate the environmental burden distribution and vulnerability to pollution sources. In close collaboration with a predominantly Latinx community in Chicago, we highlight the usefulness of our approach through a case study that shows how certain community areas in the city are likely to bear a disproportionate burden of environmental pollution caused by industrial roads.

==> review.tex <==

R1 SCORE: 0 (borderline paper)
Use of schools is an excellent study population, avoiding many of the pitfalls in more generic neighbourhoods or communities by fixing geography to a certain extent. This also perhaps limits the broader generalizability of the findings here, when exposure profiles and geographies are usually more heterogeneous. 

TODO: Some discussion of this limitation needed (or why it is not a limitation) - given concerns re: Uncertain Geographic Context Problem and other recent discussions of issues/difficulties in making place-based environmental risk associations. 

DONE
The use of ‘number of hazardous sources’ as the hazard indicator is fairly crude, essentially treating all hazards as the same and temporally homogeneous, when in reality they likely differ substantively across a profile of relevant factors (e..g, size, traffic density, timing of high traffic, etc.) which would impact actual hazard risk?

It is not totally clear what the novel contribution here is. 
What would this method get you in terms of understanding that more standard metrics such as a Bivariate local Moran’s I or even a simple correlation of spatially-derived variables (e.g., \% students vs. total kilometres per unit) achieve?

if the community-based nature of the dashboard development is the key feature here, it is not reported what that engagement achieved? What changed as a result of community input, or how community input led to the final product?

parcent > percent

%%%%%%%%%%%%%%%%%

R2 SCORE: 2 (accept)

My only two suggestions for immediate improvements are:

 - The choice of the 1-mile radius needs justification, and consideration should be given to a more appropriate distance measure that reflects the movements of the school pupils, like x minutes walking distance.

 - I wasn't quite sure why the results were aggregated to community areas at all (e.g. eq. 2). The authors could consider aggregating to a regular grid in a similar manner to calculating a Kernel Density Estimation, or something similar. Although the comparison to aggregation at the census tracts level goes some way to reduce the impact of the MAUP.


%%%%%%%%%%%%%%%%%%%%

R3 
SCORE: 2 (accept)
----- TEXT:

The type of hazardous sources is introduced late in the paper and it is difficult to understand what are you referring to in the first two pages. Also, I would call it industrial roads burden from the beginning so it is clear for the reader. If I read environmental burden I am thinking of a composite measure.

You mentioned collaborations with the Latinx communities. Would this only be for the visual aspect of the dashboard or also for the type of indexes and elements they want to be calculated for the maps and graphics?

Figure 2 includes blue circles which are difficult to understand. Maybe you could change the legend to only 2-3 categories? The upper two categories are very similar when checking the map. On another note, this can be a bit misleading because we do not know how many schools are in a community region. If there are five schools in a community region, then your 50\% let’s say would mean more exposed students than considering one school in another community region. However, representing the number of schools can make the map too full.

Figure 3: the industrial corridors and community areas have the same symbol in the legend and it makes it difficult to distinguish on the maps.

Are all the students categorized based on their ethnicity? I was wondering if there is a large number that does not declare it.

You are mentioning that MAUP and the fact that is not changing your major conclusion. Although this may be true, I would argue that it depends on the level of detail -- i.e. if you consider walking isochrones around a school, the values can change.   

Are you planning on creating a composite measure for environmental issues?

Are you considering other minorities for the exposure metric?

Would your approach be easily reproduced in other areas (cities, countries)?

Additionally, there are some small spelling errors that the authors should consider (e.g., “parcent” on page 4 second paragraph of the case study).
